Study of Peer-to-Peer Network Based Cybercrime Investigation: Application on Botnet Technologies

The scalable, low overhead attributes of Peer-to-Peer (P2P) Internet protocols and networks lend themselves well to being exploited by criminals to execute a large range of cybercrimes. The types of crimes aided by P2P technology include copyright infringement, sharing of illicit images of children, fraud, hacking/cracking, denial of service attacks and virus/malware propagation through the use of a variety of worms, botnets, malware, viruses and P2P file sharing. This project is focused on study of active P2P nodes along with the analysis of the undocumented communication methods employed in many of these large unstructured networks. This is achieved through the design and implementation of an efficient P2P monitoring and crawling toolset. The requirement for investigating P2P based systems is not limited to the more obvious cybercrimes listed above, as many legitimate P2P based applications may also be pertinent to a digital forensic investigation, e.g, voice over IP, instant messaging, etc. Investigating these networks has become increasingly difficult due to the broad range of network topologies and the ever increasing and evolving range of P2P based applications. In this work we introduce the Universal P2P Network Investigation Framework (UP2PNIF), a framework which enables significantly faster and less labour intensive investigation of newly discovered P2P networks through the exploitation of the commonalities in P2P network functionality. In combination with a reference database of known network characteristics, it is envisioned that any known P2P network can be instantly investigated using the framework, which can intelligently determine the best investigation methodology and greatly expedite the evidence gathering process. A proof of concept tool was developed for conducting investigations on the BitTorrent network.

==> ch5experimentation.tex <==
% !TeX spellcheck = en-GB
% !TeX root = thesis.tex

\chapter{Experimentation and Results}
\label{ch:experimentation}

\section{Documented P2P Network Investigation (BitTorrent)}
\label{ch4:documentedinvestigation}

The increase in popularity of peer-to-peer file distribution is well documented since the late 1990's. In 2004, all peer-to-peer traffic was measured to account for 80\% of all internet traffic and in 2005, specifically BitTorrent traffic accounted for over 60\% of the world's internet usage. [CITE BITTORRENT TRAFFIC MEASUREMENTS AND MODELS] This paper presents the results of an investigation conducted on the top 100 largest BitTorrent swarms over the course of one week. The purpose of this investigation is to determine where Each IP address discovered over the course of the week is found in a geolocation database, which results in the ability to determine exactly where the participation in these networks is prominent worldwide. This paper assumes that the reader is somewhat familiar with how content is distributed through BitTorrent.

\section{Introduction}
\label{ch4:introduction}
By the nature of the implementation of the protocol, when a peer wishes to acquire a particular piece of content, he must identify another peer in the same BitTorrent swarm who has that piece of content and is willing to share it with him.

%\begin{figure}
%\centering
%\includegraphics[width=0.98\textwidth]{images/simple.pdf}
%\caption{Fundamental design of the RAFT system.}
%\label{fig:simple}
%\end{figure}

In this paper, we present the results of an investigation to quantify the scale and distribution of the top 100 most active torrents.

\subsection{Selecting the Top 100}
The most popular BitTorrent tracking website, according to Alexa, is The Pirate Bay \cite{piratebay}. In January 2010, The Pirate Bay held the Alexa global traffic rank of number 99 and is the 91st most popular website visited by the United States \cite{alexa}. For the purposes of the investigation outlined in this paper, the top 100 torrents listed on The Pirate Bay were chosen to be monitored.


\section{Specifications of the Investigation}
The investigation was designed to connect to The Pirate Bay and download the top 100 torrents each day. These torrent swarms were then monitored for a 24 period, before the process repeated itself.The investigation was conducted using a single dedicated server. The server

The specification of the investigation was:
\begin{enumerate}
\item Connect to The Pirate Bay and download the ``.torrent'' metadata files for the top 100 torrents
\item Connect to each swarm sequentially and identify each of the peers currently active in the swarm until the total number of peers collected matched the most recent number of active peers reported by the tracker.
\item Once the active peers were found for the entire 100 torrent swarms, the process was repeated for the next 24 hours.
\item After 24 hours, the process was begun again at step 1.
\end{enumerate}

\subsection{Investigation Methodology}
For a regular BitTorrent user, the starting point to acquiring whatever content is desired is to visit a BitTorrent indexing website, e.g., The Pirate Bay \cite{piratebay}. The indexing site serves as a directory for the user of all the content available to him. The user finds the specific content he is interested in by browsing the website or through keyword searching. He must then download the ".torrent" metadata file which contains information specific to the content desired such as name, size, filenames, tracker information, hash value for completed download, chunk size, hash values for each chunk etc. This ".torrent" file is then opened with a BitTorrent client, e.g., Azureus, $\mu$Torrent etc., which in turn contacts the tracker for a bootstrapping list of a number of IP addresses to get started in the swarm.

The methodology used in this investigation to gather information involved the amplification of this regular client usage in order to collect the complete list of peers involved in any given swarm as efficiently as possible. For example, in a large swarm of 50,000 peers, the tool developed and used for this experiment is capable of collecting the active peer information in as little as 8 seconds. However, the precise design and specifications of the software used is beyond the scope of this paper.

\subsection{Assumptions}
There are a number of assumptions which had to be made for the purposes of the investigation. These assumptions had to be made for various technical limitations, such as:
\begin{enumerate}
\item That for the week long duration of the investigation, each IP address found to be participating in the swarms investigated is only ever allocated to one peer. While dynamic IP address allocation may result in the same user being allocated two or more IP addresses during the investigation, it was deemed technically infeasible to identify precisely when this may occur on a global level.
\item That the country, city and ISP level geolocation databases used are as accurate as is possible to determine. In January 2010, MaxMind claim that their GeoLite databases they provide are 99.5\% accurate at a country level, 83\% accurate at a US city level within a 25 mile radius and 100\% accurate at the ISP level \cite{maxmind}.
\item That no anonymous proxy servers or Internet Anonymity services, e.g., Tor \cite{tor}, I2P \cite{i2p}, etc., are used by the peers discovered.
\item That each IP address represents a single user at a given computer. Multiple users sharing a single computer or internet connection cannot be accounted for using the information discovered during the investigation.
\item That it is infeasible for users on dial-up internet connections to download the file size typically distributed via the BitTorrent protocol. The average file size
\end{enumerate}

\subsection{Verification of Results}
To verify that each peer discovered has one or more chunks of the content being distributed in the swarm, the crawler would have to download at least one chunk from each peer and compare the hash of this chunk with the hash supplied in the torrent metadata file.

\subsection{Forensic Integrity}


\section{Results and Analysis}
Over the week long investigation, the total number of peers discovered exceeded X.Y million.

\subsection{Top 100 Content Information}

\begin{table}
\begin{center}
\caption{Breakdown of Top 100 ``.torrent'' metadata files.}
\begin{tabular}{ l | c | c | c}

\textsc{ } & \textsc{Maximum} & \textsc{Minimum} & \textsc{Average} \\
\hline
Content Size			& 38.37Gb & 109.69Mb & 1.62Gb \\
\hline
Chunk Size          	& 4Mb & 128Kb & 1.3Mb \\
\hline
Number of Chunks           	& 19,645 & 346 & 1,251 \\
\hline
Number of Files           	& 322 & 2 & 24 \\
\hline
Number of Trackers           	& 57 & 4 & 20 \\
\hline
\end{tabular}
\label{tab:top10countries}
\end{center}
\end{table}

\subsection{Geospatial Analysis}
For each IP address discovered during the investigation, the geolocation was found using MaxMind's GeoIP databases \cite{maxmind}, which resulted in information such as 
\begin{table}
\begin{center}
\caption{Number of Broadband Subscriptions discovered during the investigation (assuming a negligible amount of dial-up users).}
\begin{tabular}{ l | p{2.7cm} | p{2.6cm} | p{2.6cm}}

\textsc{Country} & \textsc{Number of Peers Discovered} & \textsc{Broadband Subscription Count} \cite{itu} & \textsc{Percentage of Broadband Subscriptions Discovered} \\
\hline
United States			& 1,116,111 & 73,123,400 & 1.53\% \\
\hline
United Kingdom          	& 790,162 & 17,276,000 & 4.57\% \\
\hline
India           	& 549,514 & 5,280,000 & 8.70\% \\
\hline
Canada           	& 443,577 & 9,842,300 & 4.51\% \\
\hline
Spain           	& 397,848 & 8,995,400 & 4.42\% \\
\hline
Italy           		& 378,892 & 11,283,000 & 3.36\% \\
\hline
Brazil           	& 320,829 & 10,098,000 & 3.18\% \\
\hline
Australia           	& 261,433 & 5,140,000 & 5.09\% \\
\hline
Poland           	& 248,731 & 4,792,600 & 5.19\% \\
\hline
Romania           	& 215,403 & 2,506,000 & 15.4\% \\
\hline
\end{tabular}
\label{tab:top10countries}
\end{center}
\end{table}

\subsection{Peer Information Analysis}

The time taken to capture a snapshot of the 100 swarms investigation varied from hour to hour due to the increase and decrease in the overall size of the swarms. The average time to get one snapshot of each of the 100 swarms was

\begin{table}
\begin{center}
\caption{Total time that each peer was detected in one or more swarms.}
\begin{tabular}{ l | c}

\textsc{Number of Peers} & \textsc{Connection Time}\\
\hline
12121212			& $<$ 1 \nicefrac{1}{2} Hours \\
\hline
12121212			& 1 \nicefrac{1}{2}-3 Hours \\
\hline
12121212			& 3-6 Hours \\
\hline
12121212         	& 6-12 Hours \\
\hline
12121212        	& 12-24 Hours\\
\hline
12121212           	& 1-2 Days\\
\hline
1212121           		& 2-3 Days \\
\hline
121212           	& 3-4 Days \\
\hline
12121          	& 4-5 Days \\
\hline
1212           	& 5-6 Days \\
\hline
121           	& 6-7 Days \\
\hline
12           	& Entire 7 Days \\
\hline
\end{tabular}
\label{tab:top10countries}
\end{center}
\end{table}

%\section{Conclusion and Future Work}

%\begin{enumerate}
%\item \emph{Overcome DHCP Issues} - Dynamic address allocation - identification of peers through meta data and heuristic approaches.
%\item \emph{Conduct a larger scale analysis} -
%\end{enumerate}

%\section{About the Authors}

%Mark Scanlon currently is a research Ph. D. candidate in Computer Science at University College Dublin, under the guidance of Prof. Mohand-Tahar Kechadi in the UCD Centre for Cybercrime Investigation. He received his B.A. degree in Computer Science and Linguistics in 2006 and his research M.Sc. in 2009, both from University College Dublin. His research interests include Computer Forensics and Cybercrime Investigation, Networking and Internet/Peer-to-Peer protocols. \\Contact:
%\email{mark.scanlon@ucd.ie}

%Mohand-Tahar Kechadi is a Professor of Computer Science at University College Dublin. His research interests include Grid Computing and Grid Software, Distributed Data Mining on Grid Platforms and Data Mining in Digital Forensics and Cybercrime investigations. \\Contact:
%\email{tahar.kechadi@ucd.ie}

%
% ---- Bibliography ----
%

%\begin{thebibliography}{4}

%\bibitem{3g} Dahlman, E., Ekstr\"om, H., Furusk\"ar, A., Jading, Y., Karlsson, J., Lundevall, M., Parkvall, S.: The 3G Long-Term Evolution -- Radio Interface Concepts and Performance Evaluation.
%In: 63$^{rd}$ IEEE Vehicular Technology Conference, Melbourne, Australia (May 2006)

%\bibitem{alexa} Alexa Information on The Pirate Bay, Downloaded January 2010, http://www.alexa.com/siteinfo/thepiratebay.org

%\bibitem{i2p} I2P - The Anonymous Network, http://www.i2p2.de

%\bibitem{itu} International Telecommunication Union, United Nations, Report on Internet , Report Generated January 2010, http://www.itu.int

%\bibitem{maxmind} MaxMind Inc., GeoLite Country Database, Downloaded January 2010, http://www.maxmind.com


%\bibitem{gao} Gao, Y., Richard III, G.G., Roussev, V.: Bluepipe: A Scalable Architecture for On-the-Spot Digital Forensics.
%In: International Journal of Digital Evidence, vol. 3 no. 1 (2004)

%\bibitem{4g} Govil, J., Govil, J., An Empirical Feasibility Study of 4G's Key Technologies.
%In: Proceedings IEEE International Conference on Electro/Information Technology (EIT), pp. 267--270 (2008)

%\bibitem{ray} Ray, I., Shenoi, S., Advantages in Digital Forensics IV, Chapter 26: Time Analysis of Hard Drive Imaging Tools, pp. 340 -- 343 (2008)

%\bibitem{richard} Richard III, G.G., Roussev, V., Next-Generation Digital Forensics. Communications of the ACM, vol. 49 no. 2, pp. 76 -- 80 (2006)

%\bibitem{roussev} Roussev, V., Richard III, G.G., Breaking the performance wall: the case for distributed digital forensics.
%In: Proceedings of the 2004 Digital Forensics Research Workshop, Baltimore, Maryland, USA (DFRWS August 2004)

%\bibitem{sealey} Sealey, P., Remote Forensics.
% In: Digital Investigation vol. 1 no. 4, pp. 261--265. Elsevier (2004)

%\bibitem{speedtest} Speedtest Mini, Downloaded April 2009, http://www.speedtest.net/mini.php

%\bibitem{piratebay} The Pirate Bay, World's Largest BitTorrent Tracker, Total Top 100, Downloaded January 2010, http://thepiratebay.org/top/all

%\bibitem{tor} The Tor Project, http://www.torproject.org/

%\bibitem{ubuntu} Ubuntu Linux 8.04, November 2008, http://www.ubuntu.com

%\bibitem{wang} Wang, S-J., Measures of retaining digital evidence to prosecute computer-based cyber-crimes.
%In: Computer Standards \& Interfaces, vol. 29 no. 2, pp. 216-223 (February 2007)

%\end{thebibliography}
%
%\end{document}


\section{Undocumented P2P Investigation (Zeus Botnet)}
\label{c4:undocumentedinvestigation}

\section{Introduction}
\label{c4:intro}

\subsection{Selecting the botnet for investigation}
\label{c4:botnetselection}

\section{Specifications}
\label{c4:botnetspecifications}

\subsection{Investigaton Methodology}
\label{c4:botnetinvestigationmethodology}

\subsection{Assumptions}
\label{c4:botnetassumptions}

\subsection{Verification of Results}
\label{c4:botnetverification}

\subsection{Forensic Integrity}
\label{c4:botnetintegrity}

\section{Results and Analysis}
\label{c4:botnetresults}

\subsection{Gathered Information}
\label{c4:gatheredinformation}

\subsection{Geospatial Analysis}
\label{c4:geospatialanalysis}

==> ch6forensicinvestigationofzeus.tex <==
% !TeX spellcheck = en-GB
% !TeX root = thesis.tex

\chapter{Forensic Investigation of the Zeus Botnet [60]}
\label{ch6forensicinvestigationofzeus}

Irrespective of what Peer-to-Peer network is being investigated, there is a uniform methodology for its investigation. Due to the commonality of every P2P network design requiring there to be a method of joining the network and discovering other peers, a method to receive commands or queries and a process for command execution, a common investigative process can be designed. The proposed solution outlined in \ref{methodology} outlines this five step process.

\section{Investigation Methodology}
\label{methodology}

\begin{enumerate}
\item Assess -- Discover as much as possible about the network to be investigated. This can be achieved through the network sniffing of an active node in the network, e.g. deployed as part of a honeypot. Although the amount known at the end of this step will be network dependent, an ideal scenario would result in the following characteristics being known:
\begin{itemize}
\item Topology of the network
\item Protocols employed
\item Method of encryption (if any)
\item Common commands and queries available
\item Peer discovery methods
\end{itemize}
\item Develop -- This include the development of a P2P client emulator for the specific network being investigated. This client must have the ability to bootstrap onto the network while appearing as a regular node to every other active node on the network. Regular client operations must also be available, including peer discovery and peer communication.
\item Monitor -- The monitoring of the network over a specified time period will record the number of active peers, the network churn rate, the network reliability and uptime, the resource size available and the commands and queries received.
\item Analyse -- The data gathered from the monitoring step must be analysed to determine the following:
\begin{itemize}
\item The types of cybercrimes the network is being used for.
\item Any inherent weaknesses in the network such as a single point of failure or the possibility of issuing commands to the network.
\item Encryption methods employed
\item If it is possible to identify the source of the commands. This will include the identification of "super peers", i.e., nodes responsible for distributing the commands across the network and the possible identification of the controlling machine or bot master.
\end{itemize}
\item Results -- The results from this investigation will be enable law enforcement to investigate crimes on the Internet that may be otherwise going under their radar. Any reporting on the investigation should clearly explain the complete methodology of the investigation should the results be required for court proceedings.

\end{enumerate}

\section{Enhancements}
\label{enhancements}

Due to the aforementioned commonality of the design and implementation of P2P networks, it is conceivable that a P2P network investigation tool could be built that given any active P2P network node, would have the ability to automatically determine much of the networks topology, protocols and available commands. This would greatly speed up the first two steps outlined above and enable the monitoring procedures to commence as early as possible in the investigation.

\section{Documented Network Methodology}
\label{ch3:documented}
\subsection{BitTorrent Methodology}
\label{ch3:BitTorrent}


\begin{table}[!t]
\renewcommand{\arraystretch}{1.3} 
\caption{Sample Network Profile} 
\label{sampleprofile} 
\centering 
\begin{tabular}{|c|c|} 
\hline 
\bfseries Feature & \bfseries Value\\ 
\hline\hline 
fileSharing & true\\ 
\hline 
botnet & false\\ 
\hline 
centralised & true\\ 
\hline 
decentralised & true\\ 
\hline
configFile & true\\ 
\hline
encrypted & false\\ 
\hline
httpPeerDisc & true\\ 
\hline
httpFreq & 0\\ 
%\hline
%httpFormat & \$httpURL\$?param\&param\\ 
\hline
peerExchange & true\\ 
\hline
peerExchangeFreq & 300\\ 
\hline
dht & true\\ 
\hline
dhtFreq & 0\\ 
%\hline
%dhtFormat & \$httpURL\$?param\&param\\ 
\hline
%1.0 & 2.0\\ 
%\hline
\end{tabular} 
\end{table} 

To start, the basic profile for BitTorrent was recorded in the network database, as can be seen in Table \ref{sampleprofile}. Alongside this identifying information, the format of the communication methods are also stored, as can be seen in Table \ref{sampleformat}. A hierarchical object oriented approach to network investigation was implemented for each of the BitTorrent peer communication methods. In testing the crawler, it was found that by employing a hierarchical approach facilitated much of the job organisation and data processing.

\section{Undocumented Network Methodology}
\label{ch3:undocumented}
\subsection{Zeus Methodology}
\label{ch3:zeus}

==> methodology.tex <==
% !TeX spellcheck = en-GB
% !TeX root = thesis.tex

\chapter{Methodology}
\label{ch3:methodology}

Irrespective of what Peer-to-Peer network is being investigated, there is a uniform methodology for its investigation. Due to the commonality of every P2P network design requiring there to be a method of joining the network and discovering other peers, a method to receive commands or queries and a process for command execution, a common investigative process can be designed. The proposed solution outlined in \ref{methodology} outlines this five step process.

\section{Investigation Methodology}
\label{methodology}

\begin{enumerate}
\item Assess -- Discover as much as possible about the network to be investigated. This can be achieved through the network sniffing of an active node in the network, e.g. deployed as part of a honeypot. Although the amount known at the end of this step will be network dependent, an ideal scenario would result in the following characteristics being known:
\begin{itemize}
\item Topology of the network
\item Protocols employed
\item Method of encryption (if any)
\item Common commands and queries available
\item Peer discovery methods
\end{itemize}
\item Develop -- This include the development of a P2P client emulator for the specific network being investigated. This client must have the ability to bootstrap onto the network while appearing as a regular node to every other active node on the network. Regular client operations must also be available, including peer discovery and peer communication.
\item Monitor -- The monitoring of the network over a specified time period will record the number of active peers, the network churn rate, the network reliability and uptime, the resource size available and the commands and queries received.
\item Analyse -- The data gathered from the monitoring step must be analysed to determine the following:
\begin{itemize}
\item The types of cybercrimes the network is being used for.
\item Any inherent weaknesses in the network such as a single point of failure or the possibility of issuing commands to the network.
\item Encryption methods employed
\item If it is possible to identify the source of the commands. This will include the identification of "super peers", i.e., nodes responsible for distributing the commands across the network and the possible identification of the controlling machine or bot master.
\end{itemize}
\item Results -- The results from this investigation will be enable law enforcement to investigate crimes on the Internet that may be otherwise going under their radar. Any reporting on the investigation should clearly explain the complete methodology of the investigation should the results be required for court proceedings.

\end{enumerate}

\section{Enhancements}
\label{enhancements}

Due to the aforementioned commonality of the design and implementation of P2P networks, it is conceivable that a P2P network investigation tool could be built that given any active P2P network node, would have the ability to automatically determine much of the networks topology, protocols and available commands. This would greatly speed up the first two steps outlined above and enable the monitoring procedures to commence as early as possible in the investigation.

\section{Documented Network Methodology}
\label{ch3:documented}
\subsection{BitTorrent Methodology}
\label{ch3:BitTorrent}

\section{Undocumented Network Methodology}
\label{ch3:undocumented}
\subsection{Zeus Methodology}
\label{ch3:zeus}

==> progress.tex <==
\chapter{Progress to Date}
\label{ch:progress}

The Investigation Methodology outlined in \ref{methodology} was implemented to investigate a documented Peer-to-Peer network, as outlined in \ref{bttop100} below. This skills and experience from proof of concept investigation can then be built upon to investigate undocumented networks, e.g., botnets.

\section{BitTorrent Investigation}
\label{bttop100}

\begin{figure}[htb]
\centering
\includegraphics[width=0.9\textwidth]{images/categorydistribution}
\caption{Category distribution of the top 100 torrents on The Pirate Bay}
\label{fig:cat}
\end{figure}

From the analysis of the daily top 100 swarms, video content was found to be the most popular being distributed over BitTorrent. Movie and television content amounted for over 94.5\% of the total, as can be seen in Figure \ref{fig:cat}, while music, games and software amounted for 1.8\%, 2.5\% and 1.2\% respectively. One highly probable explanation for the popularity of television content is due to the lag between US television shows airing in the US and the rest of the world. 

\subsection{Geolocation and Visualisation}
\label{geolocation}

There are a number of assumptions that had to be made for the purposes of the geolocation of the IP addresses and for the count of the total number of BitTorrent users involved in the swarms investigated:
\begin{enumerate}
\item The country, city and ISP level geolocation databases used are as accurate as possible. In January 2010, MaxMind state that their geolocation databases are 99.5\% accurate at a country level, 83\% accurate at a US city level within a 25 mile radius and 100\% accurate at the ISP level \cite{maxmind}.
\item For a week long investigation, each IP address found to be participating in the swarms investigated is assumed to only ever be allocated to one end user. Due to a typical DHCP lease from an Internet service provider lasting somewhere in the order of 2-7 days, dynamic IP address allocation may result in the reallocation of the same IP address to two or more end users during the investigation. Should this have occurred during the investigation, it is ignored for the interpretation of the results outlined below. It is deemed technically infeasible to identify precisely when this may occur on a global level within the scope of this paper.
\item No anonymous proxy servers or Internet anonymity services, e.g., I2P \cite{i2p}, Tor \cite{tor}, etc., are used by the IP addresses discovered.
\item It is practically infeasible for users on dial-up Internet connections to download the very large file that typically justifies distribution via the BitTorrent protocol. The average content size for the swarms investigated was 1.62GB, which would take a typical 56kbps dial-up user over 69.5 hours to download, assuming no other Internet traffic and achieving the maximum theoretical dial-up connection speed. For the purposes of the analysis presented in section III below, it was assumed that a negligible amount of dial-up users participate in the BitTorrent swarms.
\end{enumerate}

For each IP address detected during the investigation, the geolocation is obtained using MaxMind's GeoIP databases \cite{maxmind}, which results in information such as city, country, latitude, longitude, ISP, etc., being resolved. This information is then gathered and plotted as a heatmap to display the distribution of the peers involved in copyright infringement on a world map, seen in Figure \ref{fig:heatmap}. The most popular content tends to be content produced for the English speaking population, which is reflected in the heatmap, i.e., countries with a high proportion of English speaking population are highlighted in the results.

\begin{figure}[htb]
\centering
\includegraphics[width=1\textwidth]{images/worldmap}
\caption{Heatmap showing the worldwide distribution of peers discovered}
\label{fig:heatmap}
\end{figure}

\subsection{Results}
Over the week long investigation, the total number of unique IP addresses discovered was 8,489,287. On average, each IP address detected was active in 1.75 swarms, or, almost three out of every four IP addresses were active in at least two of the top 100 swarms during the week. The largest swarm detected peaked at 93,963 active peers and the smallest swarm shrunk to just 1,102 peers. The time taken to capture a snapshot of 100 swarms investigated varies due to the increase and decrease in the overall size of the swarms. The average time to collect all the peers' information for each swarm is 3.4 seconds.

\begin{figure}[htb]
\centering
\includegraphics[trim = 0mm 5mm 0mm 0mm, clip, width=0.5\textwidth]{images/ireland}
\caption{Geolocation of the peers found across Ireland}
\label{fig:mainlandus}
\end{figure}

\begin{figure}[htb]
\centering
\includegraphics[width=0.45\textwidth]{images/uk}
\caption{Geolocation of the peers found across the United Kingdom}
\label{fig:uk}
\end{figure}

\begin{figure}[htb]
\centering
\includegraphics[width=0.9\textwidth]{images/mainlandus}
\caption{Geolocation of the peers found across the USA mainland}
\label{fig:ireland}
\end{figure}

The United States is the most popular country detected with over 1.1 million unique IP addresses, which accounted for 13.15\% of all the IP addresses found. While accounting for the largest portion of the results obtained in this investigation, this relatively low percentage suggests that BitTorrent has a much more globally dispersed user base in comparison to other large P2P networks. For example, a 10 day investigation conducted on the Gnutella network in 2009, it was found that ``56.19\% of all [worldwide] respondents to queries for content that is copyright protected came from the United States" \cite{hannaway}. When the IP addresses detected during this investigation are geolocated and graphed onto a map, the population centers can be easily identified, as can be seen in Figure \ref{fig:mainlandus}. The state of California accounted for 13.7\% of the US IPs found, with the states of Florida and New York accounting for 7.2\% and 6.8\% respectively.

The objective of this investigation was to attempt to identify the scale of the unauthorised distribution of copyrighted material worldwide using the BitTorrent protocol. 2.43\% of the broadband subscriber base were detected over the course of one week in the 163 torrents monitored. This number is far greater than the number of subscribers that could possibly be prosecuted for their actions. The number of end users involved in illegal downloading is undoubtedly much higher than this due to the relatively small scale of this investigation. Some network factors will also have a negative effect over the results achieved, such as two or more end-users appearing as a single Internet IP address though Internet connection sharing, proxy services, etc. \cite{sealey}.
